Measuring prominence of scientific work in online news as a proxy for impact

The impact made by a scientific paper on the work of other academics has many established metrics, including metrics based on citation counts and social media commenting. However, determination of the impact of a scientific paper on the wider society is less well established. For example, is it important for scientific work to be newsworthy? Here we present a new corpus of newspaper articles linked to the scientific papers that they describe. We find that Impact Case studies submitted to the UK Research Excellence Framework (REF) 2014 that refer to scientific papers mentioned in newspaper articles were awarded a higher score in the REF assessment. The papers associated with these case studies also feature prominently in the newspaper articles. We hypothesise that such prominence can be a useful proxy for societal impact. We therefore provide a novel baseline approach for measuring the prominence of scientific papers mentioned within news articles. Our measurement of prominence is based on semantic similarity through a graph-based ranking algorithm. We find that scientific papers with an associated REF case study are more likely to have a stronger prominence score. This supports our hypothesis that linguistic prominence in news can be used to suggest the wider non-academic impact of scientific work.

==> Prominence Paper/table2.tex <==

\begin{table*}[h!]
\small
\begin{tabular}{|p{7.5cm}|p{7.5cm}|}
\hline
\textbf{News Article First Sentences - High Semantic Similarity}                                                                     & \textbf{News Article First Sentences - Low Semantic Similarity}                                                     \\
\hline
One in three adults aged over 65 in England have difficulty understanding basic health-related information, suggests a study in the BMJ.         & Like many patient groups, the Alzheimers' Society isn't happy with the state of scientific research.. \\
\hline
Acne drug not found to increase suicide risk                                                                                         & It has all the makings of a pub quiz teaser: what do Barack Obama, Emma Watson, Jake Gyllenhaal and the British TV presenter Fiona Bruce have in common?                        \\
%\hline
%Risk of stillbirth for women sleeping on left on night before birth is half that for those who sleep in other positions, study shows  & Many would assume that the kinds of living mammals are completely known or nearly so, but they would be wrong. \\    
%\hline
%A new study suggests that many first memories are actually fictional and based on photographs and family stories. 
%&
%The Inter-Academy Panel, a network of the world's science academies including our own Royal Society, today issued a statement on synthetic biology. \\    
\hline
University College London researchers found a 3.6\% decline in mental reasoning in women and men aged 45-49.
&
Lately, it seems as if everyone is anti-antidepressants.\\
%\hline

%The giant sauropod dinosaurs such as Diplodocus and Apatosaurus are familiar thanks to their huge sizes and unique body shapes of a long neck and tail with a tiny head perched on top. 

%&

%I’m the first to admit that the "registration revolution" sounds less like a banner for reforming science and more like the march of a thousand bureaucrats, clipboards and pens at the ready. \\
%\hline

%Doctors have begun a trial of a simple saliva test that aims to spot the top 10\% of men who are most at risk of developing prostate cancer. 

%&
%Blue Planet II gave us a glimpse of the weird and wonderful life that swims and floats in the deep ocean, but what about the creatures that live beneath the ocean floor? 

%\\
\hline

\end{tabular}
\caption{Example `First Sentence' extracts that are helpful (left) and not helpful (right) for prominence task }
\label{tab:helpful-firstsent}
\end{table*}

